TESS-Keck Survey IX: Masses of Three Sub-Neptunes Orbiting HD 191939 and the Discovery of a Warm Jovian Plus a Distant Sub-Stellar Companion

Exoplanet systems with multiple transiting planets are natural laboratories for testing planetary astrophysics. One such system is HD 191939 (TOI-1339), a bright (V=9) and Sun-like (G9V) star, which TESS found to host three transiting planets (b, c, and d). The planets have periods of 9, 29, and 38 days each with similar sizes from 3 to 3.4 $R_{\oplus}$. To further characterize the system, we measured the radial velocity (RV) of HD 191939 over 415 days with Keck/HIRES and APF/Levy. We find that $M_b = 10.4 \pm 0.9 M_{\oplus}$ and $M_c = 7.2 \pm 1.4 M_{\oplus}$, which are low compared to most known planets of comparable radii. The RVs yield only an upper-limit on $M_d$ (<5.8 $M_{\oplus}$ at 2$\sigma$). The RVs further reveal a fourth planet (e) with a minimum mass of $0.34 \pm 0.01 M_{Jup}$ and an orbital period of 101.4 $\pm$ 0.4 days. Despite its non-transiting geometry, secular interactions between planet e and the inner transiting planets indicate that planet e is coplanar with the transiting planets ($\Delta$i < 10$^{\circ}$). We identify a second high mass planet (f) with 95% confidence intervals on mass between $2-11 \, M_{Jup}$ and period between 1700-7200 days, based on a joint analysis of RVs and astrometry from $Gaia$ and $Hipparcos$. As a bright star hosting multiple planets with well-measured masses, HD 191939 presents many options for comparative planetary astronomy including characterization with JWST.

==> ttvTableBJD.tex <==
\begin{table}[h!]
\footnotesize
\centering
 \caption{\textsc{Transit Mid-times}}
 \begin{tabular}{cccc}
 \hline
 \hline
& \multicolumn{1}{c}{Planet b} & \multicolumn{1}{c}{Planet c}  & \multicolumn{1}{c}{Planet d}\\
Transit \# & Mid-time (BJD) & Mid-time (BJD) & Mid-time (BJD)\\
\hline
0 & $2458715.3552 \pm 0.0023$        & $2458726.0546 \pm 0.0033$    & $2458743.5531 \pm 0.0038$ \\
1 & $-$                              & $2458754.6340 \pm 0.0028$    & $2458781.9029 \pm 0.0029$ \\
2 & $2458733.1156 \pm 0.0028$        & $2458783.2116 \pm 0.0031$    & $2458820.2645 \pm 0.0031$ \\
3 & $2458741.9962 \pm 0.0023$        & $2458811.7992 \pm 0.0031$    & $-$ \\
4 & $-$                              & $2458840.3758 \pm 0.0029$    & $2458896.9613 \pm 0.0038$ \\
5 & $2458759.7587 \pm 0.0024$        & $-$                          & $-$ \\
6 & $2458768.6376 \pm 0.0029$        & $2458897.5359 \pm 0.0038$    & $2458973.6648 \pm 0.0031$ \\
7 & $-$                              & $2458926.1168 \pm 0.0031$    & $-$ \\
8 & $2458786.3987 \pm 0.0021$        & $-$                          & \\
9 & $2458795.2825 \pm 0.0026$        & $-$                          & \\
10 & $2458804.1602 \pm 0.0026$       & $-$                          & \\
11 & $2458813.0424 \pm 0.0041$       &                              & \\
12 & $2458821.9181 \pm 0.0023$       &                              & \\
13 & $2458830.8014 \pm 0.0029$       &                              & \\
14 & $2458839.6806 \pm 0.0018$       &                              & \\
15 & $-$                             &                              & \\
16 & $-$                             &                              & \\
17 & $-$                             &                              & \\
12 & $2458875.2017 \pm 0.0018$       &                              & \\
19 & $-$                             &                              & \\
20 & $2458892.9626 \pm 0.0020$       &                              & \\
21 & $2458901.8430 \pm 0.0020$       &                              & \\
22 & $2458910.7222 \pm 0.0023$       &                              & \\
23 & $2458919.6017 \pm 0.0024$       &                              & \\
24 & $-$                             &                              & \\
25 & $-$                             &                              & \\
26 & $-$                             &                              & \\
27 & $-$                             &                              & \\
28 & $2458964.0028 \pm 0.0036$       &                              & \\
29 & $2458972.8837 \pm 0.0021$       &                              & \\
30 & $2458981.7649 \pm 0.0021$       &                              & \\
31 & $2458990.6450 \pm 0.0020$       &                              & \\
32 & $2458999.5248 \pm 0.0029$       &                              & \\
33 & $2459008.4056 \pm 0.0023$       &                              & \\
\hline
\hline
\end{tabular} \\
\footnotesize{{Expected transits which occur in data gaps are denoted by a dash.}}
\label{tbl:TTVs}
\end{table}

